Fine-Tuning is Fine, if Calibrated

Fine-tuning is arguably the most straightforward way to tailor a pre-trained model (e.g., a foundation model) to downstream applications, but it also comes with the risk of losing valuable knowledge the model had learned in pre-training. For example, fine-tuning a pre-trained classifier capable of recognizing a large number of classes to master a subset of classes at hand is shown to drastically degrade the model's accuracy in the other classes it had previously learned. As such, it is hard to further use the fine-tuned model when it encounters classes beyond the fine-tuning data. In this paper, we systematically dissect the issue, aiming to answer the fundamental question, "What has been damaged in the fine-tuned model?" To our surprise, we find that the fine-tuned model neither forgets the relationship among the other classes nor degrades the features to recognize these classes. Instead, the fine-tuned model often produces more discriminative features for these other classes, even if they were missing during fine-tuning! {What really hurts the accuracy is the discrepant logit scales between the fine-tuning classes and the other classes}, implying that a simple post-processing calibration would bring back the pre-trained model's capability and at the same time unveil the feature improvement over all classes. We conduct an extensive empirical study to demonstrate the robustness of our findings and provide preliminary explanations underlying them, suggesting new directions for future theoretical analysis. Our code is available at https://github.com/OSU-MLB/Fine-Tuning-Is-Fine-If-Calibrated.

==> math_analysis.tex <==
\section{Math}
Model output $ \arg\max_i \text{softmax}(w_i^T Ux)$ where $U$ is a learnable matrix, $w_c$ are the class-specific weights, and $x$ is the seen feature vector from last layer, all positive. 

For Softmax function and Cross-entropy loss:
\begin{align}
\hat{y}_i = \frac{\exp(w_i^T Ux)}{\sum_{k} \exp(w_k^T \cdot Ux)} \\
L = -\sum_{i} y_i \log(\hat{y}_i)
\end{align}

Derivative of $L$ with respect to $\hat{y}$:

\begin{equation}
    \frac{\partial L}{\partial \hat{y}_i} = -\frac{y_i}{\hat{y}_i} \\
\end{equation}


 Derivative of $\hat{y}_i$ with respect to $w_i^TUx$: \\
 \begin{equation}
\frac{\partial \hat{y}_i}{\partial (w_j^T Ux)} = \hat{y}_i (\mathbbm{1}[i = j] - \hat{y}_j) \\   
 \end{equation}


Derivative of $w_i^T Ux$ with respect to U: \\

\begin{equation}
  \frac{\partial (w_j^T Ux)}{\partial U} = w_{j}x^T \\
\end{equation}

Finally:

\begin{equation}
    \frac{\partial L}{\partial U} =  (\hat{y}_j - \mathbbm{1}[i = j]) w_{j} x^T
\end{equation}

Feature change for an unseen sample $x'$ after one update assuming the learning rate = 1 is 

\begin{equation}
    (\hat{y}_j - \mathbbm{1}[i = j]) w_{j}x^T x'
\end{equation}


The gradient of the cross-entropy loss $\sL$ with respect to a unseen class weight $\vw_c$, $c \in \sU$ for a seen class sample $(x_i, y_i)$ is 
\begin{gather}
    \frac{\partial \sL}{\partial \vw_c} = \bigl( \frac{Z_{c}(x)}{\sum_{i\in (\sU \cup \sY^\star)}Z_{i}(x_i)} - \mathbbm{1}[y_i = c]\bigr) f_{\theta_{\sT}}(x_i)
\end{gather}

% Given the prevalent use of ReLU as the activation function within feature extractors, $ f_{\theta_{\sT}}(x_i)$ is invariably positive. Since target training data only comprises seen class samples, $y_i = c$ is always false. Consequently, $\vw_c$ keeps being penalized throughout the training process. This continuous penalization leads to the progressive diminishment of the magnitude for the first term. 

% 4. \text{ Applying the Chain Rule:} \\
% \frac{\partial L}{\partial U_{jk}} = \sum_i \frac{\partial L}{\partial \hat{y}_i} \cdot \frac{\partial \hat{y}_i}{\partial (w_c \cdot Ux)_i} \cdot \frac{\partial (w_c \cdot Ux)_i}{\partial U_{jk}} \\
% \text{Substituting the derivatives, we get:} \\
% \frac{\partial L}{\partial U_{jk}} = \sum_i -\frac{y_i}{\hat{y}_i} \hat{y}_i (\delta_{ij} - \hat{y}_j) w_{ci} x_k \\

% \text{This gives you the gradient of the cross-entropy loss with respect to each element of the matrix } U. \\
% \text{Finally, the update for } U \text{ in gradient descent would be:} \\
% U = U - \alpha \nabla_U L \\
% \text{where } \alpha \text{ is the learning rate.}


==> new_text.tex <==
\begin{wrapfigure}{R}{0.35\textwidth}
    \centering
    %\vskip-15pt
    \includegraphics[width=\linewidth]{arxiv/figure/tsne_imagenet_r.pdf}
    \vskip-5pt
    \caption{\textbf{t-SNE (ImageNet-R)}. The FT extractor $f_{\vtheta_\sT}$ does not create an artificial margin between fine-tuning and absent classes.}
    \vskip-15pt
    \label{fig:tsne_in_r}
\end{wrapfigure}

\begin{wraptable}{R}{0.32\textwidth}
\centering
\footnotesize
\vskip-25pt
\setlength{\tabcolsep}{0.5pt}
\begin{tabular}{c|c|c|c}
    NCM  \text{Acc$_{\sU/\sU}$}           & PT & FT & \text{$\Delta$} \\
    \midrule
    IN-\{R, S\} & 40.3\%     & 61.9\%   & 21.6\%     \\
    \midrule
    VTAB            &      83.7\%         &      87.2\%    &       3.5\%     \\
    \midrule
    Office-Home       & 80.1\%     & 81.5\%   & 1.4\%     
\end{tabular}
\vskip-2pt
\captionof{table}{\textbf{NCM  \text{Acc$_{\sU/\sU}$} using the pre-trained (PT) and FT features.} FT improves the feature quality for absent classes.}
\label{tab: ncm_u_u}
\vskip-15pt
\end{wraptable}

To further understand the improved absent class accuracy $\text{Acc$_{\sU/\sY}$}(f_{\vtheta_\sT})$, we plot the t-SNE embedding \cite{van2008visualizing} in~\autoref{fig:tsne_in_r}. We find that the FT feature extractor $f_{\vtheta_\sT}$ does not superficially raise $\text{Acc$_{\sU/\sY}$}$ by creating an artificial ``margin'' between the fine-tuning and absent class features
\footnote{Doing so would shrink the label space from $\sY$ to $\sU$. We note that $\text{Acc$_{\sU/\sU}$}\geq\text{Acc$_{\sU/\sY}$}$: the former eliminates the errors of classifying unseen class samples into seen classes.} 
and destroying their semantic relationship. 
We further report the NCM accuracy of classifying absent class data into one of the absent classes, \ie, $\text{Acc$_{\sU/\sU}$}$ with $\sB=\sU$. As summarized in~\autoref{tab: ncm_u_u}, FT indeed improves the feature quality to distinguish among absent classes.


%%%%%%%%%%
\begin{wrapfigure}{R}{0.45\textwidth}
\centering
\vskip-22pt
    \includegraphics[width=1\linewidth]{arxiv/figure/cali.pdf}
    \vskip-10pt
    \caption{\small \textbf{Post-hoc calibration} with an additive $\gamma$ lifts the logits of unseen classes to reclaim correct prediction.}
    \label{fig: calibration-demo}
    \vskip-25pt
\end{wrapfigure}


%%%%%%%
\paragraph{Average logit gap (ALG).} 
The first approach estimates $\gamma$ by calculating the logit gap between seen and unseen classes, taking the insight that a calibrated model should assign logits of similar scales to non-ground-truth classes, regardless of seen or unseen. 
Since the target training data $D_\text{tr}$ contains only the seen class examples, we calculate for each 
training example 1) the average of non-ground-truth seen class logits and 2) the average of unseen class logits. We then average the difference between them over all the training examples as an estimate of $\gamma$.

%~\autoref{fig:logits} reveals that for Naive FT, the average non-GT logits are markedly higher within the seen class group compared to the unseen class group. In contrast, the source model exhibits more comparable non-GT logits between these groups. This disparity inspires a calculation of $\gamma$ based on the differential non-GT logits between seen and unseen classes, as delineated in \autoref{eq: baseline}. The entire process is visually summarized in \autoref{fig:baseline}.
\iffalse
\begin{align}
        \gamma_{baseline} = \frac{1}{|\sT|}\sum_{(x_i, y_i) \in \sT} \bigl[ &\frac{1}{|\sS|}\sum_{c \in \sS \& c \neq  y_i} \vw_{c}^{T}f_{\theta_{\sT}}(x) 
    -  \frac{1}{|\sU|}\sum_{c \in \sU \& c \neq  y_i}\vw_{c}^{T}f_{\theta_{\sT}}(x)\bigr]
    \label{eq: baseline}
\end{align}
\fi



% \begin{figure}
%     \centering
%     \includegraphics[width=0.7\linewidth]{icml2024/figure/baseline.pdf}
%     \caption{Baseline calibration method: $\gamma$ is calculated based on the differential non-GT scores between seen and unseen classes. }
%     \label{fig:baseline}
% \end{figure}

\paragraph{Pseudo cross-validation (PCV).}
The key challenge in selecting $\gamma$ stems from the absence of unseen training data, preventing us from assessing its quality in balancing between \text{Acc}$_{\sS/\sY}$ and \text{Acc}$_{\sU/\sY}$. To circumvent this, we partition the target training dataset $D_\text{tr}$ into two subsets with disjoint label spaces, simulating pseudo-seen and pseudo-unseen classes. 
We then naively fine-tune the pre-trained model on the pseudo-seen set and estimate \text{Acc}$_{\sS/\sY}$ and \text{Acc}$_{\sU/\sY}$ on both sets. This procedure enables us to select a $\gamma$ by balancing these two accuracies. (More details can be found in the Appendix.)
We repeat this process three times with different data splits to obtain a more stable, averaged estimate of $\gamma$. 


\begin{wraptable}{R}{0.35\textwidth}
\centering
\footnotesize
\vskip-15pt
\setlength{\tabcolsep}{0.5pt}
\begin{tabular}{c|c|c|c}
AUSUC    & IN-\{R, S\} & VTAB  & O-H \\
\midrule
Pre-trained   & 0.083             & 0.444 & 0.499       \\
\midrule
Tu \etal~\cite{tu2023holistic}        & 0.317             & 0.553 & 0.618       \\
\midrule
Fine-tuning & \textbf{0.439}             & 
\textbf{0.586} & \textbf{0.632} \\    
\midrule
\end{tabular}
\vskip-5pt
\caption{{Results in AUSUC.}}
\label{tab: auc}
\vskip-15pt
\end{wraptable}

\begin{figure}[t]
\centering
    \begin{minipage}[t]{0.4\linewidth}
        \centering
        \includegraphics[width=\linewidth]{arxiv/figure/3lines/3lines_imagenet_r.pdf}
        \mbox{\small (a) ImageNet-R }
    \end{minipage}%
    \begin{minipage}[t]{0.4\linewidth}
        \centering
        \includegraphics[width=\linewidth]{arxiv/figure/3lines/3lines_oh_ar_pr.pdf}
        \mbox{\small (b) Office-Home}
    \end{minipage}%
\vskip-5pt
\caption{\textbf{The Seen-Unseen Accuracy Curve} (\small \text{Acc}$_{\sS/\sY}$ at the x-axis and \text{Acc}$_{\sU/\sY}$ at the y-axis) by varying the calibration factor $\gamma$. In (b), we use the Art domain to pre-train the classifier and the Product domain as the target.}
\label{fig:AUSUC_new}
\vskip-15pt
\end{figure}

\paragraph{Why is unseen class relationship preserved?}
To elucidate the preservation of the unseen class relationship, we analyze how classifier weights $\mW$ change within the seen and unseen classes. We commence by calculating the L2 normalized weight changes between naive FT and the pre-trained model $\Delta \mW = \frac{\mW_{\sT} - \mW_{\sO}} {\lVert \mW_{\sT} - \mW_{\sO}\rVert_2}$. Visualizing the cosine similarity of the change within seen and unseen classes, \ie
$\Delta \mW^{\sY} (\Delta \mW^{\sY})^\top$ and $\Delta \mW^{\sU} (\Delta \mW^{\sU})^\top$, allows us to assess the directional similarities in classifier updates. As depicted in \autoref{fig: classifier_delta_IN}, there exists a pronounced dissimilarity in the update directions among seen classes since the gradients aim to separate seen classes during fine-tuning. Conversely, a notable similarity in the update directions is observed among unseen classes. The absence of positive signals from unseen class data results in nearly uniform updates of unseen classifiers, thereby preserving the class relationships among unseen classes throughout fine-tuning. More results for other datasets can be found in the Appendix. 
\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{arxiv/figure/classifier_delta_IN_S.pdf}
    \vskip -5pt
    \caption{\small Classifier update direction similarity within seen (left) and unseen (right) classes for ImageNet-S. The update directions are highly similar within unseen classes, thus preserving the inter-class relationships among unseen classes.}
    \label{fig: classifier_delta_IN}
    \vskip -15pt
\end{figure}




